Stochastic Krasnoselskii-Mann Iterations: Convergence without Uniformly Bounded Variance

We investigate the Stochastic Krasnoselskii-Mann iterations for expected nonexpansive fixed-point problems in a real separable Hilbert space. We establish convergence guarantees under significantly weaker assumptions on the variance than those typically used in the literature. In particular, instead of a uniform bound on the variance of the stochastic oracle, we only assume finite variance at a single fixed point. Under this assumption, we prove almost sure weak convergence of the iterates, derive convergence rates for the expected residual and the last-iterate residual, and obtain almost sure convergence rates for the running minimum residual. Notably, we recover the best-known stochastic oracle complexity without imposing uniformly bounded variance. We illustrate the applicability of our results to Stochastic Gradient Descent, where we recover known guarantees, to Stochastic Three-Operator Splitting and Stochastic Backward-Forward Splitting, for which we obtain the first results that avoid uniform variance bounds, and to a novel Stochastic Lifted Three-Operator Splitting.

==> customcommands.tex <==
% Change Log:
%   - 2026-05-15 (v2.0): Moved many commands into customarticle and custompresentation

% --- Packages ---                  % Set margins
\usepackage{parskip}                % Removes indent at start of paragraph
\usepackage[scale=2]{ccicons}
\usepackage{booktabs}
\usepackage{amsmath}
\usepackage{amssymb}            
\usepackage{graphicx}               % To import pictures
\usepackage{mathtools}              % Allows various math, such as \coloneqq
\usepackage{multicol, multirow}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{array}
\usepackage{tikz}                   % For Tikz figures
\usepackage{pgfplots}               % For PGF figures, makes Tikz easier
\pgfplotsset{compat=newest}
\usepackage{xcolor}                 % For colors
\usepackage[normalem]{ulem}         % For strikeout using \sout
\usepackage{tablefootnote}          % For footnotes in tables

% --- Custom commands ---
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\renewcommand{\H}{\mathcal{H}}

\newcommand{\Var}{\operatorname{Var}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\prox}{\operatorname{prox}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\cone}{\operatorname{cone}}
\newcommand{\interior}{\operatorname{int}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\spa}{\operatorname{span}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Zer}{\operatorname{Zer}}
\newcommand{\diam}{\operatorname{diam}}

% Specific to PIKM Project
\newcommand{\Fix}{\operatorname{Fix}}

% Specific to SGD Project
\newcommand{\Exp}[1]{\mathbb{E}\mathopen{}\left[{#1}\right]\mathclose{}}
\newcommand{\Expt}[1]{\mathbb{E}_t\mathopen{}\left[{#1}\right]\mathclose{}}
\newcommand{\ExpD}[2]{\mathbb{E}_{{#1}}\mathopen{}\left[{#2}\right]\mathclose{}}

% Specific to HVI Project
\newcommand{\Gap}[1]{\operatorname{Gap}({#1})}
\newcommand{\GapOpt}[1]{\operatorname{Gap}_{\operatorname{opt}}({#1})}
\newcommand{\GapFeas}[1]{\operatorname{Gap}_{\operatorname{feas}}({#1})}
\newcommand{\SOL}{{\operatorname{SOL}}}
\newcommand{\VI}{{\operatorname{VI}}}

% Specific to SKM Project
\newcommand{\supp}{\operatorname{supp}}
\renewcommand{\O}{{\mathcal O}}
\newcommand{\graph}{\operatorname{graph}}

% Specific to DP Project
\newcommand{\D}{{\mathcal D}}
\renewcommand{\L}{{\mathcal L}}
\renewcommand{\S}{{\mathbb S}}
\newcommand{\X}{{\mathcal X}}
\newcommand{\Y}{{\mathcal Y}}
\newcommand{\priv}{{\operatorname{priv}}}
\newcommand{\Wishart}{{\operatorname{Wishart}}}
\newcommand{\sym}{{\operatorname{sym}}}
\newcommand{\rank}{{\operatorname{rank}}}
\newcommand{\exact}{{\operatorname{ex}}}
\newcommand{\final}{{\operatorname{final}}}
\newcommand{\Jp}{{\mathcal J_\priv}}
\newcommand{\Jpi}{{\mathcal J_\priv^i}}
\newcommand{\tJp}{{\widetilde{\mathcal J}_\priv}}
\newcommand{\J}{{\mathcal J}}
\newcommand{\ran}{\operatorname{ran}}
\newcommand{\op}{\operatorname{op}}
\newcommand{\lin}{{\operatorname{lin}}}

% Specific to CNM Project
\newcommand{\slow}{{\operatorname{slow}}}
\newcommand{\fast}{{\operatorname{fast}}}
